Perceptual Quality Assessment of 360$^\circ$ Images Based on Generative Scanpath Representation

Despite substantial efforts dedicated to the design of heuristic models for omnidirectional (i.e., 360$^\circ$) image quality assessment (OIQA), a conspicuous gap remains due to the lack of consideration for the diversity of viewing behaviors that leads to the varying perceptual quality of 360$^\circ$ images. Two critical aspects underline this oversight: the neglect of viewing conditions that significantly sway user gaze patterns and the overreliance on a single viewport sequence from the 360$^\circ$ image for quality inference. To address these issues, we introduce a unique generative scanpath representation (GSR) for effective quality inference of 360$^\circ$ images, which aggregates varied perceptual experiences of multi-hypothesis users under a predefined viewing condition. More specifically, given a viewing condition characterized by the starting point of viewing and exploration time, a set of scanpaths consisting of dynamic visual fixations can be produced using an apt scanpath generator. Following this vein, we use the scanpaths to convert the 360$^\circ$ image into the unique GSR, which provides a global overview of gazed-focused contents derived from scanpaths. As such, the quality inference of the 360$^\circ$ image is swiftly transformed to that of GSR. We then propose an efficient OIQA computational framework by learning the quality maps of GSR. Comprehensive experimental results validate that the predictions of the proposed framework are highly consistent with human perception in the spatiotemporal domain, especially in the challenging context of locally distorted 360$^\circ$ images under varied viewing conditions. The code will be released at https://github.com/xiangjieSui/GSR

==> section/2_introduction_copy.tex <==
\section{Introduction}

\IEEEPARstart{V}{irtual} reality (VR) photography endeavors to capture or recreate a spherical natural scene into omnidirectional~(\ie, \omni) images. \omni images offer a vast interactive space, making them particularly appealing in the realm of metaverse applications.  
However, one of the main barriers to the broader adoption of VR photography is the significant loss of quality that \omni images undergo during the processes of image capture, projection, compression, and transmission~\cite{Sun2017_subj, Duan2018_subj}. Consequently, investigating the factors that influence the perceptual quality of \omni images has emerged as a significant research topic.

\input{figs/intro}

Researchers have devoted considerable efforts to analyzing the \textit{global} distortions that uniformly affect the quality of \omni images, such as compression, Gaussian blur, and noise~\cite{Sun2017_subj, Duan2018_subj,MC360IQA2019,VGCN2020, MultiStream2021, MFILGN2021, MPBOIQA2021, SPANet2021, Zhang2022, Yang2022, wu2023assessor360}. Numerous subjective user studies have been conducted on degraded \omni images~\cite{Sun2017_subj, Duan2018_subj, SPANet2021}, leading to the development of several objective omnidirectional image quality assessment~(OIQA) models~\cite{MC360IQA2019, VGCN2020, MultiStream2021,  MFILGN2021, SPANet2021, MPBOIQA2021, Zhang2022, Yang2022, wu2023assessor360}. A family of explicit methods aims to extend the 2D full-reference IQA model for the OIQA task~\cite{SPSNR2015,CPPPSNR2016,WSPSNR2017,SSSIM2018} by considering the stretch ratio of the equirectangular projection~\cite{CPPPSNR2016,WSPSNR2017} or the spherical properties of \omni images~\cite{SPSNR2015,SSSIM2018}. However, since comparing entire omnidirectional images is inconsistent with human perception in \omni scenes due to the limited field of view (FoV), a more effective approach is to evaluate the perceptual quality of \omni images by combining quality scores of viewport images~\cite{MC360IQA2019,VGCN2020, MultiStream2021, MFILGN2021,Sui2021,MPBOIQA2021, JUFE22, Zhang2022, Yang2022, wu2023assessor360}. 

Unfortunately, these methods largely overlook the diversity of viewing behaviors that leads to variations in the perceived quality of \omni images, as shown in  Fig.~\ref{fig:intro}~(a). This oversight manifests in two key aspects. 
First, two viewing conditions that significantly
sway user gaze patterns are frequently overlooked. 
Specifically, the \textit{starting point of viewing} and the \textit{exploration time} can significantly impact the scanpath patterns, which in turn affect the perceived quality of \omni images, particularly when images are locally distorted~\cite{Sui2021,JUFE22}. For instance, users may fail to detect distortions if they start viewing from a distortion-free area with a short exploration time. As such, the perceptual quality might vary significantly among users under different viewing conditions.
Second, the majority of OIQA methods predominantly relies on a single fixed viewport sequence from the \omni image to predict its perceptual quality, as shown in Fig.~\ref{fig:intro} (b). 
However, the deterministic quality evaluation relying on one fixed sequence cannot explain the probabilistic viewing behaviors with randomness, thereby potentially leading to prediction bias. 

Despite a few studies have attempted to address these issues~\cite{Sui2021,JUFE22,wu2023assessor360}, they still manifest certain limitations. 
Sui~\etal\cite{Sui2021} proposed an OIQA method by integrating the quality scores of multiple viewport sequences generated using human scanpaths. However, this approach poses significant computational challenges due to the necessity of extracting a multitude of viewport images.
Fang~\etal~\cite{JUFE22} introduced an OIQA model that adapts to different viewing conditions by embedding the positions of the uniformly sampled viewports and the prompts of starting point and exploration time. However, this model did not consider users' viewing behaviors that
can significantly impact the perceptual quality.
Recently, Wu~\etal~\cite{wu2023assessor360} proposed an OIQA model that incorporates a strategy for sampling multiple viewport sequences based on patch-wise entropy. However, such a method may not be adequate to model complex viewing behaviors that are impacted by a variety of factors, \eg, scene semantics and kinematic constraints~\cite{Sitzmann18}.

In this study, we introduce a novel computational framework for OIQA. The underlying principle of the framework is to infer the perceptual quality of \omni images by aggregating dynamic perceptual experiences of multi-hypothesis users. The inference process is operated under a predefined viewing condition which is characterized by the starting point and exploration time. More specifically, given an arbitrary starting point and exploration time, a set of scanpaths~\cite{scandmm2023} can be produced. This aligns with the philosophy that users' viewing behaviors exhibit significant variation due to the diversity of individual experiences and preferences~\cite{Sitzmann18,Sui2021}. 
Subsequently, the unique generative scanpath representation (GSR) is constructed by aggregating multiple small gazed-focused areas, as shown in Fig.~\ref{fig:intro} (c). 
As such, the quality inference of \omni image can be swiftly transformed to that of GSR which realistically incorporates the viewing behaviors. Our contributions are summarized as follows: 
\begin{itemize}
     \item We introduce a novel computational framework for OIQA that infers quality based on a set of realistic scanpaths generated under a predefined viewing condition. As such, we bridge the gap between viewing conditions and quality assessment in \omni scenes.
     
    \item We propose a unique GSR representation that offers a comprehensive global overview of dynamic perceptual experiences of multi-hypothesis users. As such, our framework is able to make a thorough quality assessment from a variety of experiences.  

    \item We conduct comprehensive experiments to demonstrate the effectiveness and efficiency of the proposed model. In particular, our model is much more accurate than advanced OIQA models with less computational complexity.
\end{itemize}


==> section/4_method_copy.tex <==
\section{The Proposed Computational Framework}
The framework presented in Fig.~\ref{fig:framework} consists of three components: the scanpath generator, the GSR converter, and the quality evaluator. This section first provides an overview of the rationale behind each module. Subsequently, the details of each module are discussed.

The framework is designed to adapt to a predefined viewing condition by using a scanpath generator to generate scanpaths based on a given starting point and exploration time. This allows the collection of quality opinions from multi-hypothesis users under a specific viewing condition, similar to the methodology of subjective user studies~\cite{series2012methodology,Sui2021}. To reduce the redundant calculations in quality inference for viewport images, which are caused by the high probability of overlap among the FoV of different users (see Fig.~\ref{fig:vcr} (a)), we propose to ``downscaling'' the \omni image to a GSR sequence that realistically incorporates viewing behaviors. Inspired by the visual neuroscience that visual detail is captured primarily by the fovea (\ie, the center of gaze)~\cite{ungerleider2000mechanisms}, the quality inference is conducted on the aggregation of small gaze-focused areas at each time instance (see Fig.~\ref{fig:vcr} (b)). Finally, a 3D backbone is used to extract quality-aware features from the GSR sequence, which contains spatiotemporal information of perceptual experiences, to model the temporal quality variation of perceptual experiences.

\input{figs/framework}
\subsection{Input Data}
Our computational framework takes two inputs: 1) a \omni image $\mathbf{I}$, which is in the form of 2D equirectangular projections; 2) a viewing condition $\mathbf{\Omega}=\{\mathcal{P}_1,\ T\}$ that includes a starting point $\mathcal{P}_1 = (y_1, x_1)$ and an exploration time $T$, where $(y_1, x_1)$ indicates the normalized 2D coordinate at the initial moment with values in the range of $[0, 1]$.

\subsection{Scanpath Generator}
We produce realistic scanpaths using an effective scanpath prediction model which is capable of accurately replicating human gaze behaviors. For \omni scenes, the generator should have two essential features: \begin{itemize} 
\item \textit{Adaptability}: it should be able to adapt to any predefined viewing condition, with the capacity to generate scanpaths from any starting point and for any exploration time. 
\item \textit{Generativity}: it should be consistent with probabilistic viewing behaviors, with the capacity of generating different scanpaths for a given \omni image. \end{itemize}
The \textit{adaptability} enables the framework to be relevant and effective in inferring perceptual quality by adapting to predefined viewing conditions. Furthermore, the \textit{generativity} allows for a diverse range of viewing behaviors to be taken into account for a thorough quality inference. An additional benefit of using a generative model is that the resulting scanpaths and corresponding GSR sequence can vary with each iteration, implying that new training samples can be generated regardless of data augmentation~\cite{MAE2022}. The effectiveness of such a strategy is demonstrated in Sec.~\ref{sec:abl}. In this study, we use ScanDMM~\cite{scandmm2023} as the scanpath generator within our framework. Given a \omni image $\mathbf{I}$ and viewing condition $\mathbf{\Omega}$, ScanDMM produces a scanpath through the generative process of the Markov model. This process is carried out in parallel to create $N$ plausible scanpaths: 
\begin{equation}
\begin{split}
\mathcal{\hat{P}}^{1:N}_{1:T} = \mathcal{G}(\mathbf{I}, \mathbf{\Omega}).
%&= \\&= \{(y^n_t, x^n_t)\}_{t=1}^{T}, \quad n = 1,2,...,N.
\end{split}
\end{equation}
$\mathcal{G}$ is the ScanDMM model. $\mathcal{\hat{P}}^{1:N}_{1:T} = \{\{(y^n_t, x^n_t)\}_{t=1}^{T}\}_{n=1}^{N}$ is a set of $N$ generated scanpaths, where $(y^n_t, x^n_t)$ represents the predicted gaze point of $n$-th hypothetical user at time instant~$t$. 

%it is \textit{flexible} and \textit{generative}. Specifically, it has the ability to generate a scanpath of arbitrary length from arbitrary starting point, and the capability to produce diverse scanpaths for a given \omni image.
%As such, we can obtain a variety of perceptual experiences derived from scanpaths for perceptual quality assessment of \omni images. This is consistent with the methodology of subjective user studies~\cite{series2012methodology} that collects quality opinions from multiple subjects.


% The visible content at a specific time instance could be determined by the gaze positions and a valid FoV\footnote{A typical FoV of the head-mounted displays is $90\degree\times110\degree$ along latitude and longitude directions, respectively.}. However, maintaining the entire image content within the FoV is cumbersome and redundant, as the time-consuming projection processing and the high likely overlap of FoVs of different users~(as shown in Fig.~\ref{fig:vcr}).
% In our study, inspired by the subjective user study of IQA~\cite{series2012methodology} -- gathering quality opinions from multiple subjects, we propose to approximate the \textit{global} visible content of all users\footnote{Refers to the assumed user unless otherwise specified.} by combining \textit{portions} from each FoV (as shown in Fig.~\ref{fig:vcr}). Considering the space-varying distortions inherent to equirectangular projection, we use the spherical convolution~\cite{SphereNet2018} that takes into account the stretch ratio of the equirectangular projection to extract the mini-patch on the spherical tangent domain. It enables the end-to-end model to run faster than the common approach of extracting viewports, where the coordinates are retrieved pixel by pixel through a rectilinear projection~\cite{Ye2017JVET_360Lib}. The primary factor underlying the high \textit{efficiency} of the proposed representation remains the small size of the extracted mini-patches. Until now, we provide an effective way to model the dynamic perception of multiple users, and a spatial-temporal visible content representation (VCR) representation for quality-aware feature extraction. In addition, we demonstrate such a representation can also improve full-reference OIQA metrics in Sec.~\ref{sec:exp_vcr}.

 %Furthermore, except for constructing a robust blind OIQA model with VCR, we demonstrate that such a representation can also enhance the performance of full-reference OIQA metrics in Sec.~\ref{sec:exp_vcr}.
%This approach enables the end-to-end model to run more efficiently than the existing method of extracting viewports,
%This approach provides us with a high \textit{efficiency} efficient end-to-end training model without extracting the entire viewport image by retrieving coordinates pixel-by-pixel through rectilinear projection~\cite{Ye2017JVET_360Lib}. 
%The primary factor underlying the high \textit{efficiency} of the proposed representation is the small size of the extracted mini-patches. 


%To be specific, given a predicted gaze position as the center, we extract a mini-patch with a small size of $(h, w)$ from the image $\mathbf{I}$ using spherical convolution. 

% Herein, we introduce the details about the process of converting a \omni image into a VCR sequence. We first create a kernel pattern for spherical convolution.
% Let $\mathcal{S}$ be the unit sphere and $\mathcal{T}(\phi, \theta)$ be the tangent plane located at $\mathcal{S}(\phi, \theta)$, where $\phi\in[-\frac{\pi}{2}, \frac{\pi}{2}]$ and $\theta\in[-\pi, \pi]$ represent the latitude and longitude, respectively. We create a kernel pattern $\mathbf{K}$ on tangent plane $\mathcal{T}(0, 0)$ via the gnomonic projection~\cite{map_project, SphereNet2018}:
% \begin{align}
%     &\mathbf{K}(0, 0) = (0, 0), \\
% &\mathbf{K}(i, 0) = ( 
% \mathrm{tan}(i*\Delta\phi),\ 0), \\
% &\mathbf{K}(0,  j) = (0,\ \mathrm{tan}(j*\Delta\theta)), \\
% &\mathbf{K}(i, j) = (\mathrm{tan}(i*\Delta\phi) * \mathrm{sec}(i*\Delta\theta),\  \mathrm{tan}(j*\Delta\theta)),
% \end{align}
% where $i$ and $j$ are integers that range from $[-\frac{\mathbf{P}_h}{2}, \frac{\mathbf{P}_h}{2}]$ and $[-\frac{\mathbf{P}_w}{2}, \frac{\mathbf{P}_w}{2}]$, respectively, for a patch size of $(\mathbf{P}_h, \mathbf{P}_w)$. $ \Delta\phi=\frac{\pi}{\ \mathbf{I}_h}$ and $\Delta\theta=\frac{2\pi}{\ \mathbf{I}_w}$ are the sampling step sizes that are determined by the size of image $\mathbf{I}$. 


% Given a specific gaze point $\mathcal{\hat{P}}=(\Hat{y}, \Hat{x})$ (the subscripts are omitted here for simplicity), we first convert the 2D plane coordinate $(\Hat{y}, \Hat{x})$ to its spherical coordinate $\mathcal{S}(\Hat{\phi}, \Hat{\theta})$. Then, we apply the filter $\mathbf{K}$ at its location $\mathcal{S}(\Hat{\phi}, \Hat{\theta})$ to obtain the sampling points on the sphere domain by the inverse gnomonic projection~\cite{map_project}:
% \begin{equation}
% \begin{split}
% \phi(i, j) &= \sin^{-1}(\cos v\sin \Hat{\phi}+\frac{\mathbf{K}(i,\bullet)\sin v \cos \Hat{\phi}}{\rho}), \\
% \theta(i, j) &= \Hat{\theta} + \tan^{-1}(\frac{\mathbf{K}(\bullet,j)\sin v}{\rho \cos \Hat{\theta} - \mathbf{K}(i,\bullet)\sin \Hat{\theta} \sin v}),
% \end{split}
% \end{equation}
% where $\rho=\lVert \mathbf{K}(i,j)\rVert_2$ and $v=\tan^{-1}\rho$. $\mathbf{K}(i,\bullet)$ and $\mathbf{K}(\bullet,j)$ are equal to $\mathrm{tan}(i*\Delta\phi) * \mathrm{sec}(i*\Delta\theta)$ and $\mathrm{tan}(j*\Delta\theta)$, respectively. 
% Finally, the spherical coordinates of the sampling points are projected back to 2D plane so that we can access the pixel values.
\subsection{GSR Converter}

\input{figs/vcr} 

Herein, we detail the process of converting a \omni image into a GSR sequence using the generated scanpaths. Given a predicted gaze position as the center, we extract a mini-patch with a small size of $(\mathbf{P}_h\times \mathbf{P}_w)$ from the image. To account for the overstretch inherent in the equirectangular projection, the patch extraction process is executed using the spherical convolution~\cite{SphereNet2018} which adaptively wraps the kernel around the sphere (see Fig.~\ref{fig:framework} (c)). More specifically, the spherical convolution retrieves the spherical coordinates of sampling points by using a kernel created on the spherical tangent domain. Then, these spherical coordinates are projected to the 2D plane to access the pixel values. 
By repeating the patch extraction process over each hypothetical user, a set of $N$ mini-patches can be obtained at each time instance. These patches are subsequently organized to construct a GSR sequence (denoted as $V_{1:T}$), where each GSR consists of $\sqrt{N}$ rows and columns of patches (see Fig.~\ref{fig:vcr} (b)). Additionally, to capture the temporal quality variation of the independent mini-patch sequence, we impose a constraint on their positions to ensure alignment across time, as suggested in~\cite{wu2022fastquality}. This is done as if an individual mini-patch sequence were a mini-video.

\subsection{Quality Evaluator} 
Our approach presents \omni images using GSR sequences, which contain essential spatiotemporal information of perceptual experiences for quality inference. %Different from the study~\cite {Sui2021} that predicted the quality score of the \omni image by applying a 2D-IQA method to viewport sequences, 
As such, we leverage an advanced backbone network in video tasks to learn spatiotemporal quality of the GSR sequences. 
Overall, with the resulting GSR sequence of a \omni image, we maximize the following likelihood function:
\begin{equation}
\boldsymbol{\alpha}^* = \arg\max_{\boldsymbol{\alpha}} p(q | \mathcal{M}(\mathcal{Q}(V_{1:T})); \mathbf{\boldsymbol{\alpha}}), 
\end{equation}
where $q$ is the ground-truth quality score and $\boldsymbol{\alpha}$ denotes the learnable parameters in the network.  $\mathcal{Q}$ and $\mathcal{M}$ are the quality evaluator and Multilayer perceptron (MLP) layer, respectively.
The quality inference of the \omni image is achieved by entering the GSR sequence into the quality evaluator and the MLP layer:
\begin{equation}
    \hat{q} = \mathcal{M}(\mathcal{Q}(V_{1:T})),
\end{equation}
where the $\hat{q}$ is the predicted quality score. In this study, we use the X-Clip-B/32~\cite{XCLIP2022} as the quality evaluator. The last MLP layer of X-Clip-B/32 is substituted with the one tailored for video quality assessment~\cite{wu2022fastquality}. We refer to the proposed model as GSR-X. 

%The specific backbone and MLP layer tested in this study are introduced in Sec.~\ref{sec:method_models}.


% \subsection{Specific Models}
% \label{sec:method_models}
% \begin{algorithm}[t]
% \caption{The generative process of ScanDMM. Note that ``$\sim$'' denotes the sample operation and $\mathcal{P}_t$ is the ground-truth gaze point at time instance $t$.}
% \label{alg:scandmm}
% \textbf{Input:} \\
% 1) The \omni image $\mathbf{I}$; \\
% 2) The viewing conditions $\mathbf{\Omega}=\{\mathcal{P}_1, T\}$. \\
% \textbf{Output:} \\
% Plausible scanpaths $\mathcal{\hat{P}}_{1:T}$. 
% \begin{algorithmic}[1]
% \State $\mathcal{H}_1 \leftarrow f(\mathcal{P}_1)$ \Comment{Initialize hidden state } 
% \For{$t \leftarrow 1$ to $T$}
%     \State $\mathcal{H}_t \sim p(\mathcal{H}_t|\mathcal{H}_{t-1}, \mathbf{I})$ \Comment{Transition probability}
%     \State $\hat{\mathcal{P}}_t \sim p(\mathcal{P}_t|\mathcal{H}_t)$  \Comment{Emission probability}
% \EndFor
% \State \textbf{end for}
% \end{algorithmic}
% \end{algorithm}
% \subsubsection{Scanpath generator}
% In this study, ScanDMM~\cite{scandmm2023} is employed as the scanpath generator. Given a \omni image $\mathbf{I}$ and viewing condition $\mathbf{\Omega}$, ScanDMM produces a scanpath through the generative process of the Markov model. This process is carried out in parallel to create $N$ plausible scanpaths: 
% \begin{equation}
% \begin{split}
% \mathcal{\hat{P}}^{1:N}_{1:T} = \mathcal{G}(\mathbf{I}, \mathbf{\Omega}).
% %&= \\&= \{(y^n_t, x^n_t)\}_{t=1}^{T}, \quad n = 1,2,...,N.
% \end{split}
% \end{equation}
% $\mathcal{G}$ is the ScanDMM model. $\mathcal{\hat{P}}^{1:N}_{1:T} = \{\{(y^n_t, x^n_t)\}_{t=1}^{T}\}_{n=1}^{N}$ is a set of $N$ generated scanpaths, where $(y^n_t, x^n_t)$ represents the predicted gaze point of $n$-th hypothetical user at time instant~$t$. 

% \vspace{4pt}
% \subsubsection{Quality Evaluator}
% We construct several examples of using the popular 3D backbone as the quality evaluator in our proposed framework:
% \begin{itemize}
%     \item Video Swin-T~\cite{SwinT3D2022}, the spatiotemporal adaptation of Swin Transformer~\cite{Swin2021}, extends the scope of local attention computation from the spatial domain to the spatiotemporal domain.
%     \item ConvNeXts-T~\cite{ConvNet2022}, the pure convolutional neural network, reconstructs ResNet-50 toward the design of the hierarchical vision Transformer~\cite{Swin2021}. ConvNeXts re-highlights the importance of convolutions in computer vision.
%     \item X-Clip-B/32~\cite{XCLIP2022}, the extension of Clip~\cite{clip2021} for video domains, provides a cross-frame attention strategy for the temporal modeling of videos. X-Clip has shown great effectiveness in video recognition.
% \end{itemize}
% The suffixes of the models indicate the particular variants. We substitute the last MLP layers of these backbones with the one tailored for video quality assessment~\cite{wu2022fastquality}. We refer to the proposed framework with different quality evaluators as VCR-S, VCR-C, and VCR-X, which correspond to the Swin-T, ConvNetXts-T, and X-Clip-B/32 backbones, respectively.

==> section/8_bio.tex <==
\newpage

\section{Biography Section}
If you have an EPS/PDF photo (graphicx package needed), extra braces are
 needed around the contents of the optional argument to biography to prevent
 the LaTeX parser from getting confused when it sees the complicated
 $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
 your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
 simpler here.)
 
\vspace{11pt}

\bf{If you include a photo:}\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}

\vspace{11pt}

\bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiographynophoto}{John Doe}
Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
\end{IEEEbiographynophoto}

==> tab/speed.tex <==
\begin{table*}[htb]
\small
\renewcommand\arraystretch{1.2}
\tabcolsep=0.05cm
\centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\caption{Efficiency comparison in the case of predicting a \omni image with a resolution of $4$K, $8$K, and $11$K, respectively. The values are in seconds. Our framework operates $10$-$1000$ times faster than the advanced models.}
\begin{threeparttable}
\begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}l|lll|lll|lll@{}}
\toprule[0.4mm]
&  \multicolumn{3}{c|}{$4$K}  & \multicolumn{3}{c|}{$8$K} & \multicolumn{3}{c}{$11$K} \\
Method & Preprocessing & Inference & Total & Preprocessing & Inference & Total & Preprocessing & Inference & Total \\
\hline
MC360IQA~\cite{MC360IQA2019} & $613.057$ & $11.110$ & $624.167$ & $2585.009$ & $20.657$ & $2605.666$ & $5319.346$ & $46.997$ & $5366.343$\\
%MFILGN~\cite{MFILGN2021} & 28.427 & 0.310 & 28.737 & 122.040 &  & & 238.868 & 0.848 & 239.716 \\
Fang22~\cite{JUFE22} & $19.117$ & $3.754$ & $22.871$ & $81.424$ & $3.784$ & $85.208$ & $157.656$ & $4.340$ & $161.996$ \\
VGCN~\cite{VGCN2020} & $3.364$ & $3.913$ & $7.277$ & $4.244$ & $3.940$ & $8.184$ & $4.435$ & $3.936$ & $8.371$ \\
Assessor360~\cite{wu2023assessor360} & - & $4.307$ & $4.307$ & - & $4.741$ & $4.741$ & - & $4.518$ & $4.518$ \\
CEOIQA-X & -  & $0.754$ & $\mathbf{\underline{0.754}}$ & - & $0.765$ & $\mathbf{\underline{0.765}}$ & - & $0.769$ & $\mathbf{\underline{0.769}}$\\

 \bottomrule[0.4mm]
\end{tabular*}
\end{threeparttable}
\label{tab:speed}
\end{table*}
